Why (and When) does Local SGD Generalize Better than SGD?

Local SGD is a communication-efficient variant of SGD for large-scale training, where multiple GPUs perform SGD independently and average the model parameters periodically. It has been recently observed that Local SGD can not only achieve the design goal of reducing the communication overhead but also lead to higher test accuracy than the corresponding SGD baseline (Lin et al., 2020b), though the training regimes for this to happen are still in debate (Ortiz et al., 2021). This paper aims to understand why (and when) Local SGD generalizes better based on Stochastic Differential Equation (SDE) approximation. The main contributions of this paper include (i) the derivation of an SDE that captures the long-term behavior of Local SGD in the small learning rate regime, showing how noise drives the iterate to drift and diffuse after it has reached close to the manifold of local minima, (ii) a comparison between the SDEs of Local SGD and SGD, showing that Local SGD induces a stronger drift term that can result in a stronger effect of regularization, e.g., a faster reduction of sharpness, and (iii) empirical evidence validating that having a small learning rate and long enough training time enables the generalization improvement over SGD but removing either of the two conditions leads to no improvement.

==> exper.tex <==
\section{Experiments}

\kaifeng{change it to a experiment setup section}

In this section, we conduct experiments on CIFAR-10 and ImageNet to verify that our theory can indeed lead to correct predictions to practice.
\kaifeng{TBA}

\subsection{Local SGD with label noise}

\begin{comment}
First, we focus on the case of training overparameterized neural nets with label noise regularization,
where the limiting SDEs of the standard SGD and Local SGD in the late phase
have simple forms and can be understood easily.
The label noise regularization is a simple technique
that works by flipping the target label

for the standard SGD,
the limiting SDE turns out to be the following deterministic flow that keeps reducing the trace of Hessian:
%becomes deterministic and has a simple form:
%In this special case, the limiting SDE of the standard SGD
%becomes deterministic and has a simple form:
%turns out as the following deterministic flow that keeps reducing the trace of Hessian:
\begin{align}
    \dd \vzeta(t) = -\frac{c_0}{4B} \gradGa \tr(\nabla^2 \cL(\vzeta)) \dd t,
    \label{eq:flow-label-noise-std}
\end{align}
where $\gradGa f$ stands for the gradient of a function $f$ projected to the tangent space of $\Gamma$.
As the trace of Hessian can be seen as a measure for the sharpness of the local loss landscape,
we can then see
from \eqref{eq:flow-label-noise-std} 
that SGD in this case has an implicit bias toward flatter minima,
which presumably promotes generalization.
%The relationship between sharpness and generalization has been studied in \citep{???} \kaifeng{add some discussion}
%which presumably promotes generalization~\citep{?}

We can firmly demonstrate the benefits of Local SGD
in terms of accelerating this process of sharpness reduction.
Note that $B = K \Bloc$ for Parallel SGD with $K$ workers and $\Bloc$ samples per local batch.
As $K$ increases, the speed of sharpness reduction slows down.
However, if Parallel SGD is used instead of Parallel SGD,
the limiting SDE becomes
\begin{align}
\nabla\left(\frac{1}{2H\eta} \tr (F(2H\eta \nabla^2\cL(\vzeta) ))\right)
\end{align}


In this special case,
the noise covariance matrix is a constant multiple of the Hessian at each global minimizer,
i.e., $\mSig(\vtheta^*)=c_0\nabla^2 \cL(\vtheta^*)$ for some $c_0 > 0$.
Previous works~\citep{???} have thus shown that the limiting SDE of the standard SGD
turns out to have a simple form:

%and without any data augmentation.
In this special case,
i.e., for some constant $c_0$, it holds for all global minima $\vtheta^*$ that

\end{comment}

%In this subsection, 
First, we conduct experiments for Local SGD with label noise regularization on non-augmented CIFAR-10 dataset.
As discussed in \Cref{sec:thm label noise}, in the label noise setting, the limiting SDE turns out as a simple form
and has a bias toward flatter minima,
which presumably promote generalization.
This bias is further amplified as the number of local steps $H$ increases.
%\citep{blanc2020implicit, damian2021label, li2021happens}
% and converges as $H$ goes to infinity.
See Figure \xinran{TBA} for the test accuracy on VGG-16 \citep{DBLP:journals/corr/SimonyanZ14a} without normalization  and ResNet-56 with GroupNorm.

% the assumptions of our theorem are likely to hold. 



In our experiments, we set the corruption probability $p$ to $0.1$, and run Local SGD with $32$ workers, where the local batch size of each client is $\Bloc=128$ (so the total batch size is $B = 4096$).
All workers are initialized at a common starting point, which is generated by running Parallel SGD with the same batch sizes until a high training accuracy is reached.
%batch size $4096$, and the corruption probability $p$ is set to $0.1$. We simulate 32 workers with $\Bloc=128$
%and all workers initialize at the same point near the manifold of minimizers. 
To ensure smoothness of the training loss, we use mean pooling in VGG-16 and Swish \citep{ramachandran2017searching} activation for both architectures.
At each local update, each client samples a mini-batch from the whole dataset with replacement, following our theoretical setup.
We set the learning rate $\eta$ as $0.1$ and $0.05$ for ResNet-56 and VGG-16 respectively. We train the model until the test accuracy plateaus. See \Cref{sec:label noise detail} for more implementation details.


\subsection{Generalization Benefit of Reducing the Diffusion}
As our theory suggests, when the number of local steps $H$ is large, Local SGD has the same drift term as small-batch SGD but reduces the diffusion term. In this subsection, we show empirically that this reduction of diffusion is beneficial to generalization.  We train ResNet-56 with various numbers of workers $K$ on augmented CIFAR-10 dataset for $H=600$. As illustrated in Figure \xinran{TBA} and Table \xinran{TBA}, a higher test accuracy is achieved as $K$ increases. Moreover, this generalization benefit saturates as $K$ exceeds some threshold.

The training procedure is  summarized as follows and we refer to the readers to \xinran{TBA} for full details. We first run small-batch SGD with batch size $128$ and learning rate $\eta=0.5$ for $250$ epochs to obtain the common initialization. Resuming from epoch $250$ with $\eta=0.05$, we run Local SGD with $K=16$ until epoch $6000$ and run all other setups for the same number of iterations (See Figure \xinran{TBA}). To get closer to the manifold \xinran{can we say "manifold" here? Because it may not exist}, for each setup, we continue to train with standard SGD using $\eta=0.005$ while keeping the total batch size unchanged. We report the test accuracy when the training loss drops down to $4\times 10^{-4}$ in \Cref{table:diffusion}.

\begin{table}[H]
\centering
\caption{Diffusion reduction. Average over three runs}
 \begin{tabular}{|l|c|}
 \hline
$K$ & Test acc. (\%)\\
  \hline
  $1$ & $94.5_{\pm 0.1}$ ($94.50_{\pm 0.11}$)\\
  $2$ & $94.7_{\pm 0.0}(94.73_{\pm 0.03})$\\
  $4$ & $94.7_{\pm 0.1}(94.68_{\pm 0.09})$\\
  $8$ & TBA\\
  $16$ & TBA\\
\hline
 \end{tabular}
 \label{table:diffusion}
\end{table}

%When training a model for multi-class classification on dataset $\{(\vx_i, \vy_i)\}_{i=1}^{N}$, adding label noise means 
\subsection{Momentum? (if time \& space allowed)}


\begin{comment}
\subsection{Plan (old)}
%In this section, validate our theory and discuss to what extent our theory holds through extensive experiments.
%in the late phase of training?

%We only compare $H=1$ v.s. $H > 1$ and keep the total batch size fixed.
Settings:
\begin{enumerate}
     \item Standard training setting: CIFAR-10 with augmentation, ImageNet.
    \item Non-augmented CIFAR-10 with label noise : In this setting, the manifold exists. The Hessian matrix and noise covariance satisfy $\nabla^2\cL(\vphs)=c\mSig(\vphs)$. The limiting flow has a simple form, which implies a sharpness reduction bias. 
    \item About the effect of the diffusion term: CIFAR-10 with augmentation.   Fix the number of updates and using the same learning rate schedule as small-batch SGD. Set a relatively large $H$. As $K$ increases (fix $\Bloc$ and therefore total batch size$B$ increases), the diffusion term decreases, which may help generalization.
    \item When the each client keeps a partition of the whole dataset and data is never shuffled across workers,  Local SGD is still better
    \item Local SGDm is also better than SGDm. (Be careful with the correct way to add momentum, e.g., average both param and momentum? use SlowMo?)
    %Phenomenon: Adding momentum greatly accelerates and stabilizes training
\end{enumerate}
\end{comment}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old-intro.tex <==
\section{Old Introduction}
\kaifeng{TBA}

\kaifeng{===== old intro =====}

%In the special case of $H = 1$, this can be shown to be equivalent to Parallel SGD, assuming neither has a momentum term.


This generalization benefit of Local SGD was first observed by \cite{lin2020dont}
They focused on Local SGD with a particular type of NLS schedule, named Post-Local SGD.
This algorithm  starts with standard SGD and adds local steps in the late phase of training, i.e., when the training accuracy is already high.
Extensive experiments were further conducted to show the superiority of Post-Local SGD in terms of generalization.

%reduce the communication cost.
%We can also adjust the number of local steps according to a schedule (called NLS schedule). \xinran{is this name ok?  be careful about motivation. emphasize somewhere that this is a theoretical paper; not a system paper} 
% system concern? emphasize theoretical in the title

Empirical evidence abounds that Local SGD attains higher test accuracy than standard SGD within a fixed wall-clock time budget because Local SGD reduces the frequency of communication \citep{yu2019parallel, lin2020dont, wang2019adaptive}. However, the convergence of Local SGD is slower \xinran{cite a lot of papers} when we fix the number of epochs. Intuitively, the reason is that local stochastic gradients are no longer the unbiased estimator of the full-batch gradient at the global iterate. Despite higher training error, 
Local SGD surprisingly exhibits better generalization performance than the standard SGD, if an appropriate NLS schedule is applied to Local SGD.
This generalization benefit of Local SGD was first observed by \cite{lin2020dont} \xinran{Homegeneous case. All workers have access to the whole dataset. Local SGD with shuffling. }. They focused on Local SGD with a particular type of NLS schedule, named Post-Local SGD. This algorithm  starts with standard SGD and adds local steps in the late phase of training, i.e., when the training accuracy is already high. Extensive experiments were further conducted to show the superiority of Post-Local SGD in terms of generalization.
Our experiments confirm that increasing the number of local steps in the late phase of training helps generalization. See \Cref{fig:acc} and \Cref{table:acc}.

%Besides, we observe that increasing that in early phases of training also helps generalization. 
%With an appropriate NLS schedule, Local SGD can even exhibit better generalization performance than standard SGD. 
%As shown in , Local SGD consistently outperforms standard SGD for various numbers of local steps. 
%its SGD counterpart with the same total batch size.
%through extensive expriements.
%  achieves significantly better generalization performance than large-batch SGD./
%\paragraph{Why good unclear.} 

Existing theoretical analysis of Local SGD is mainly
restricted to the optimization perspective. Adding local
steps degrades the convergence rate. \xinran{cite a lot of papers}

\kaifeng{this paragraph contains too much details; will be moved to a later section}
In terms of generalization, \cite{lin2020dont} provided an informal explanation that adding local steps injects ``well-structured''
noise to the SGD training dynamics,
which encourages convergence to flatter minima and better generalization. But they did not define the term ``well-structured'' precisely,\xinran{too detailed} and instead they illustrated the intuition that the smaller batch size used in the local updates
amplifies the gradient noise.
However, it is still unclear how this noise amplification helps generalization,
 since these local updates are just intermediate steps for updating the global iterate.
 At the end of each round, the aggregation step averages the local iterates over all workers, which may cancel out the noise amplification effect. Thus, there is a lack of theoretical understanding of how Local SGD promotes generalization. 
%\xinran{Actually, we did not explain why }
%in the sense that Local SGD better mimics small-batch SGD.

\kaifeng{why not traditional SDE approximation?}\xinran{Kaifeng check this paragraph} This paper provides a theoretical
explanation for the generalization benefit of Local SGD in the sense that it better mimics the behavior of small-batch
SGD. Specifically, we mathematically characterize the limiting dynamics of Local SGD via stochastic differential
equations (SDEs). SDE approximation of optimization algorithms is a widely used methodology \citep{hu2017diffusion,
li2019stochastic, malladi2022sdes, li2021validity} which enables researchers to analyze the optimization trajectory from
a continuous perspective without losing the inherent stochasticity. Let $\eta$ be the learning rate and the conventional
SDE approximation of SGD over $\cO(\eta^{-1})$ time is:
%This methodology has been widely used and the conventional SDE approximation of SGD over $\cO(1/\eta)$ time has the following form:
\begin{align}
    \dd\vX(t)=-\nabla \cL(\vX)\dd t+\sqrt{\frac{\eta}{B}}\mSig^{1/2}(\vX)\dd \vW(t), \label{eq:canonical SDE 2}
\end{align}
where $\vW(t)$ is the standard Wiener process and $B$ is the total batch size. However, SDEs of this type fail to separate Local SGD from standard SGD in the late phase of training when the learning rate is small (see \Cref{thm:small thm}). An intuitive explanation is that the stochastic term in \eqref{eq:canonical SDE} becomes negligible when $\eta$ goes to zero and $B$ is fixed. In this case, both algorithms closely track gradient descent for $\cO(\eta^{-1})$ time. Instead, we follow the framework proposed by \cite{li2021happens} and capture the dynamics of the projection of the global iterate on the manifold of minimizers, which lasts for 
$O(\eta^{-2})$ time.
\subsection{Our Contributions}
\kaifeng{large batch then small batch?}
\kaifeng{Our Contributions (draft):}
\xinran{We study the with replacement case}
\begin{enumerate}
    \item We explicitly characterize the dynamics of Local SGD in the late phase of training. We show that when $\bvths[s]$ reaches
a point near the manifold of minimizers of $\Gamma$, it will stay close to the manifold
and its projection on the manifold approximately tracks an SDE (\Cref{sec:theory}).
% \xinran{better sell.} 
\item The theory indicates that Local SGD better mimics the behavior of small-batch SGD.
%, match our intuition, provide rigorous, sound, intuitive explanation for the generalization benefit.\xinran{we did not explain why it generalizes better actually.}
\item We verify our theory experimentally. \kaifeng{TBA}
\item We provide a practical guidance ? 
%on how to set the number of local steps. \xinran{not sure}
\item Discuss other settings, momentum, heterogeneity, early phase of training.
\end{enumerate}

\kaifeng{Issues:}
\begin{enumerate}
    \item How to analyze the early phase (or provide a stronger argument showing that the late phase is more important)? Or should we claim that we analyze Post-Local SGD?
    \item We find a paper \citep{ortiz2021trade} aruging that post-local SGD is less effective on ImageNet. We suspect:
    \begin{enumerate}
        \item The switching point is not late enough. In Figure 7 of their paper, switching standard SGD to local SGD at epoch 60 indeed improves generalization (90 epochs in total).        \item They are doing Local SGD with momentum (Local SGDm), but the momentum term is not synchronized in the aggregation step. The momentum term may need to be handled more carefully so that Local SGDm outperforms standard SGDm. In their paper, they show that SlowMo outperforms standard SGDm, where SlowMo is Local SGDm with an additional momentum term for global updates~\citep{wang2019slowmo}.
        \item Their batch size is 2048 and not large enough. There is only a minor performance gap between large-batch training with batch size $\le 8192$ and small-batch training with $256$ \citep{goyal2017accurate}.
    \end{enumerate}
    We will run experiments on ImageNet to see what happens.
     \item About the practical guidance:  increase the number of local steps for smaller LR.  Keep $\eta H$ constant to obtain consistent performance. (e.g., for cosine learning rate schedule, use larger $H$ for smaller $\eta$. When tuning $H$, we should search at the magnitude of at least $\cO(1/\eta)$. The superiority of Post-Local SGD comes from the interplay of $\eta$ and $H$. If we keep $H$ fixed and decay the learning rate, the generalization benefit diminishes. )
     \item The combination of normalization and weight decay. Consider the training loss $\cL(\vtheta)=\hat{\cL}(\vtheta)+\frac{\lambda}{2}\normtwo{\vtheta}^2$, where $\hat{\cL(\vtheta)}$ is scale invariant. Then all minimizers of $\cL(\vtheta)$ form a cone. Among these minimizers, the point with smaller norm gives smaller value of $\cL$. Therefore, the training loss does not have a manifold. How to deal with this case? Zhiyuan's new paper: analyze the dynamics around the minimizer manifold of $\hat{\cL}$. Actually, when combined with normalization, the role of weight decay is to accelerate the limiting diffusion (exponentially fast than without weight decay)
\end{enumerate}



\begin{figure}[htb!]
\vspace{-0.15in}
\begin{center}
    \subfigure[ Accuracy on training set]{
        \includegraphics[width=0.4\textwidth]{figs/train_accv2.pdf}\label{fig:new_a}
        \hspace{-0.01in}
    }
    \subfigure[ Test accuracy ]{
        \includegraphics[width=0.4\textwidth]{figs/test_acc.pdf}\label{fig:new_b}
        \hspace{-0.01in}
    }
    \vspace{-0.01in}
    \caption{\xinran{TBA} Adding local steps in the late phase of training helps generalization.( Select one run each setting for visualization, shuffle the dataset across all workers at each epoch.  $H_1\to H_2$ means the training starts with $H_1$ local steps and switches to $H_2$ in when the learning rate decays.)}
        \label{fig:acc}
    \vspace{-0.15in}
\end{center}
\end{figure}
\begin{table}[H]
\centering
\caption{Adding local steps in the late phase of training helps generalization. (Setting: CIFAR-10 with data augmentation, ResNet-56 with BN, $\Bloc=128$, $K=32$, $KB=4096$ 500 epochs, 
shuffle every epoch, mean and standard deviation across 5 runs. BN statistics are calculated by passing $8$ batches before evaluation.
 warmup epochs 50. Do not add weight decay to BN parameters. $H_1\to H_2$ means the training starts with $H_1$ local steps and switches to $H_2$ in when the learning rate decays. small-batch baseline acc: $94.26_{\pm 0.11}$)}
 \xinran{$H_1=1, H_2=24$}
 %switch to
 \begin{tabular}{|l|c|}
 \hline
 Local steps& Test acc (\%)\\
  \hline
  $H=1\to 1$ & $91.39_{\pm 0.31}$ \\
    $H=1\to 24$ & $92.57$\\
    $H=1\to 120$ & $92.99$\\
    $H=1\to 600$ & $92.32$\\
  $H=2\to 2$ & $92.43_{\pm 0.14}$\\
  $H=2\to 24$ & $\mathbf{93.21}_{\pm 0.05}$ \\
  $H=2\to 120$ & $93.13$ \\
  %$H=2\to 96$ & $93.01_{\pm 0.24}$\\
  $H=2\to 600$ & $92.86_{\pm 0.11}$\\
\hline
 \end{tabular}
 \label{table:acc}
\end{table}

\begin{table}[H]
\centering
\caption{Experiments for Local SGD with momentum}
 \begin{tabular}{|l|c|}
 \hline
 Local steps& Test acc (\%)\\
  \hline
  $H=1\to 1 \to 1$ & $93.45_{\pm 0.24}$ \\
  $H=1\to 24 \to 24$ & $93.9_{\pm 0.23}$\\
  $H=1\to 24\to 900$ & $\mathbf{94.0}_{\pm 0.05}$\\
  $H=2\to 2 \to 2$ & $93.5_{\pm 0.24}$\\
  $H=2\to 24 \to 900$ & $93.8_{\pm 0.24}$\\
\hline
 \end{tabular}
 \label{table:acc momentum}
\end{table}


Old section 4:
\kaifeng{mention \citep{wang2019adaptive}? maybe not}

==> old-thm.tex <==

\begin{definition}[Slow SDE for Local SGD]
Given $\eta, H > 0$ and $\vzeta_0 \in \Gamma$, define $\vzeta(t)$ as the
solution of the following SDE with initial condition $\vzeta(0) = \vzeta_0$:
\begin{align}\label{eq:oldzeta}
    \dd \vzeta(t)=\frac{1}{\sqrt{B}}\partial \Phi(\vzeta)\mSig^{1/2}(\vzeta)\dd \vW(t)+\frac{1}{2B}\partial^2 \Phi(\vzeta)\left[\mSig(\vzeta) + (K-1) \mPsi(\vzeta)\right]\dd t.
\end{align}
%\kaifeng{make it self-contained; $\mSig$ noise covariance}
Here, $\mPsi(\vzeta)\in \R^{d \times d}$ is defined as follows:
\begin{align*}
      \mPsi(\vzeta) = \sum_{1 \le i, j \le d} \psi(\eta H\cdot (\lambda_i + \lambda_j)) \left\langle\mSig(\vzeta), \vv_i \vv_j^\top \right\rangle \vv_i \vv_j^\top,
\end{align*}
where 
$\{\vv_i\}_{i=1}^{d}$ is a set of eigenvectors of $\nabla^2 \cL(\vzeta)$
that forms an orthonormal eigenbasis, 
$\lambda_1,\dots,\lambda_d$ are the corresponding eigenvalues.
Additionally, $\psi(0) = 0$ and $\psi(x):=\frac{e^{-x}-1+x}{x}$ for $x \ne 0$.
\end{definition}
\begin{remark}
Intuitively, $\mPsi(\cdot)$ rescales the entries of the noise covariance in the
eigenbasis of Hessian. In the special case where
$\nabla^2\cL(\vtheta)=\diag(\lambda_1, \cdots, \lambda_d) \in \R^{d \times d}$, we have $\Psi(\mSig_0)_{i, j} =
\psi(\eta H (\lambda_i + \lambda_j)) \Sigma_{0, i, j}$.
$\psi(x)$ is a
monotonically increasing function, which goes to $1$ as $x$ goes to infinity and
approaches $0$ as $x$ approaches $0$ (see \Cref{fig:psi}).
\end{remark}
\begin{remark}
    
which equals $\Phi(\zeta + \mA \dd \vW_t + \vb \dd t) - \Phi(\zeta)$ by Itô calculus.
\end{remark}

\begin{wrapfigure}{r}{0.33\textwidth}
    \centering
    \includegraphics[width=0.3\textwidth]{figs/psi.pdf}
    \caption{A plot of $\psi(x)$}
    \label{fig:psi}
\end{wrapfigure}


We call this SDE as the ``Slow'' SDE for Local SGD because we will show that
each discrete step of Local SGD corresponds to a continuous time interval of
$\eta^2$ instead of an interval of $\eta$ in the conventional SDE. In this
sense, our SDE is ``slower'' than the conventional SDE (and hence is able to
track a longer horizon). This Slow SDE is inspired by \citet{li2021happens}.
Under nearly the same set of assumptions, \citet{li2021happens} proved that SGD
can be tracked by~\eqref{eq:zeta} with $K=1$, i.e., with the $(K-1)\Psi(\vzeta)$
term dropped. We refer to their SDE as the {\em Slow SDE for SGD}. This key
difference between our SDE and theirs is the main novelty of our theoretical
analysis, and should be the key to separate the generalization behaviors of
Local SGD and SGD in theory. We will discuss this point later in \Cref{subsec:impl}.

Now we present our SDE approximation theorem for Local SGD.
\begin{theorem}\label{main thm: flow} Let Assumptions~\ref{a:smooth} to
 \ref{a:compact} hold. Let $T>0$ be a constant and $\vzeta(t)$ be the solution
 to \eqref{eq:zeta} with the initial condition $\vzeta(0)=\Phi(\bvths[0])\in
 \Gamma$. If $H$ is set to $\tfrac{\alpha}{\eta}$ for some constant $\alpha >
 0$, then for any $\cC^3$-smooth function $g(\vtheta)$,
 $\max_{0\leq s \leq \frac{T}{H\eta^2}}\left \lvert\E[g(\Phi(\bvths)] - \E[g(\vzeta(sH\eta^2)]\right\rvert=\ctO(\eta^{0.25})$, where $\ctO(\cdot)$ hides log factors and constants
 that are independent of $\eta$ but can depend on $g(\vtheta)$.
\end{theorem}
\begin{remark}
The theorem only requires the gradient flow projection of the initial point to
be in $\Gamma$ and allows the initial point to be arbitrarily far from $\Gamma$,
which means it can be applied to random initialization as long as the
gradient flow starting from it converges to $\Gamma$.
\end{remark}


The above theorem suggests that the trajectories of the manifold projection and
the solution to the Slow SDE~\eqref{eq:zeta} are close to each other in the
sense of weak approximation.
This measurement of closeness between the iterates
of stochastic gradient algorithms and their SDE approximations is also adopted
by~\citet{li2019stochastic,li2021validity,malladi2022sdes}, but their analyses
are for conventional SDEs.

It is worth to note that the proof technique for the above theorem is novel and
is significantly different from \citet{li2021validity}. Their analysis of the
Slow SDE approximation for SGD proceeds by invoking Katzenberger's theorem with
advanced stochastic calculus. They proved that the discrete algorithm converges
to the Slow SDE in distribution but without any quantitative error bounds.
However, our proof only uses relatively simpler mathematics, such as the method of
moments, but we are able to obtain a weak approximation error rate
$\ctO(\eta^{0.25})$.


The following theorem further states that the iterate $\bvths$ will keep close
to its manifold projection after first few rounds. It also clearly exhibits the
dependency of the closeness on $\alpha:=H\eta$ and explains the reason why the
test accuracy can degrade for relatively large $\eta$ and $H$ in Figure TBA.
%, indicating that increasing $H$ for fixed $\eta$ negatively affects the quality of approximation.
% $\{\Phi(\bvths)\}_{s=0}^{\floor{T/(H \eta^2)}}$ is a near order-$0.25$ weak approximation of $\{\vzeta(t)\}_{t=0}^T$.
%\xinran{The test functions are bounded on the manifold.}



%The following theorem indicates that $\bvths$ stays within $\ctO(\sqrt{\eta})$ from the manifold after $\cO(\log \frac{1}{\eta})$ rounds with high probability.
% \begin{theorem}\label{thm:x}
% For $\delta=\cO(\poly(\eta))$, with probability at least $1-\delta$, for all $\cO(\log\frac{1}{\eta})\leq s\leq\floor{T/(H\eta^2)} $, 
%  \begin{align*}
%     \Phi(\bvths)\in \Gamma, \qquad \normtwo{\bvths-\Phi(\bvths)}=\cO\left(\sqrt{\eta \log \frac{1}{\eta\delta}}\right),
%  \end{align*}
%  where $\cO(\cdot)$ hides constants independent of $\eta$ and $\delta$.
% \end{theorem}

%The following corollary sheds light on how $\alpha$ affects the approximation error.
\begin{theorem}
\label{coro:alpha}
    For $\delta=\cO(\poly(\eta))$, with probability at least $1-\delta$, for all $\cO(\frac{1}{\alpha}\log\frac{1}{\eta})\leq s\leq\floor{\frac{T}{\alpha\eta}} $, 
    $\Phi(\bvths)\in \Gamma$ and $\normtwo{\bvths-\Phi(\bvths)}=\cO(\sqrt{\alpha\eta \log \frac{\alpha}{\eta\delta}})$,
 where $\cO(\cdot)$ hides constants independent of $\eta$, $\alpha$ and $\delta$.
\end{theorem}

\subsection{Interpretation of Slow SDEs} \label{subsec:impl}
\kaifeng{need to update}
In this subsection, we take a
closer look at the Slow SDE~\eqref{eq:zeta} to explain the role of each
component and provide important insights into why Local SGD generalizes better
than SGD. 

Setting $H=1$ in \eqref{eq:zeta},   we recover the limiting SDE for SGD with batch size $B$ in \citet{li2021happens}:
\begin{align}\label{eq:zeta-large}
    \dd \vzeta(t)=\frac{1}{\sqrt{B}}\partial \Phi(\vzeta)\mSig^{1/2}(\vzeta)\dd \vW(t)+\frac{1}{2B}\partial^2 \Phi(\vzeta)\left[\mSig(\vzeta)\right]\dd t.
\end{align}
Following \citet{li2021happens},
we can rewrite \eqref{eq:zeta-large} as following:
\begin{align}\label{eq: sde sgd}
    \dd \vzeta(t)&=P_{\vzeta}\Big(\underbrace{\frac{1}{\sqrt{B}} \partial \Phi(\vzeta) \mSig^{1/2}(\vzeta)\dd \vW(t)}_{\text{(a)\ Diffusion}}\underbrace{-\frac{1}{2B}G(\vzeta) \dd t}_{\text{(b)\ Regularization}}\Big),
\end{align}
Here $G(\vzeta):=\nabla^3\cL(\vzeta)[\cV_{\vzeta}(\mSig_{\Diamond}(\vzeta))]$,
where $\mSig_{\Diamond}(\vzeta):=\mSig(\vzeta)-\partial\Phi(\vzeta)\mSig(\vzeta)\partial \Phi(\vzeta)$
denotes the noise covariance with tangent space noise removed
(see \Cref{lemma:mani projection}).
For any differential form $\mA \dd \vW_t + \vb \dd t$,
we use $P_{\vzeta}(\mA \dd \vW_t + \vb \dd t)$ as
a shorthand for $\partial \Phi(\vzeta) \mA \dd \vW_t + \left(\partial \Phi(\vzeta) \vb + \frac{1}{2}\partial^2 \Phi_{\vzeta}[\mA \mA^\top]\right) \dd t$,
which equals $\Phi(\zeta + \mA \dd \vW_t + \vb \dd t) - \Phi(\zeta)$ by Itô calculus.
In \eqref{eq: sde sgd}, $P_{\vzeta}$ serves as a special projection operator
that keeps $\vzeta$ on the manifold $\Gamma$.


%When $\vzeta \in \Gamma$ and $\vdelta$ is small, $P_{\vzeta}(\vdelta) = \partial \Phi (\vzeta) \vdelta + \frac{1}{2} \partial^2 \Phi(\vzeta)[\vdelta \vdelta^\top]$.

%\xinran{Definition of the stochastic differential form} 

%the remaining part of the noise covariance after removing the part in the tangent space

% By \citet{li2021happens},  \eqref{eq:zeta-large} can be rewritten as:
\begin{comment}
\begin{align}\label{eq: sde sgd}
\begin{aligned}
    \dd \vzeta(t)
    &=\underbrace{\frac{1}{\sqrt{B}}\partial \Phi(\vzeta)\mSig^{1/2}(\vzeta)\dd \vW(t)-\frac{1}{2B}\nabla^2 \cL(\vzeta)^+\nabla^3 \cL(\vzeta)[\mSig_{\parallel}(\vzeta)]\dd t}_{\text{(a)\ Diffusion \ Part}}\\
    &\quad \underbrace{-\frac{1}{2B}\partial \Phi(\vzeta)\nabla^3\cL(\vzeta)[\cV_{\nabla^2 \cL(\vzeta)}(\mSig_{\Diamond}(\vzeta))]\dd t}_{\text{(b)\ Regularization\ Part}}.
\end{aligned}
\end{align}

\begin{align}
    P_{\zeta}(z) &= \Phi(\zeta + z) - \zeta \\
    P_{\zeta}\left(\frac{1}{\sqrt{B}}\mSig^{1/2}(\vzeta)\dd \vW(t) - \frac{1}{2B} \nabla^3\cL(\vzeta)[\cV_{\nabla^2 \cL(\vzeta)}(\mSig_{\Diamond}(\vzeta))]\dd t \right)
\end{align}

\begin{align}
    \dd \zeta = P_{\zeta}^*(b \, \dd t)
\end{align}
$\Phi^*_{\vzeta}(\frac{1}{\sqrt{B}}\mSig^{1/2}(\vzeta)\dd \vW(t))$
$\Phi_z$ function

$\Phi_z^*$ $\sigma dW + b dt \rightarrow \sigma' dW + b' dt$
\end{comment}
 For the limiting SDE of Local SGD, we take $\alpha$ to infinity to simplify the SDE and obtain a similar form:
 \begin{align}\label{eq: sde local sgd}
    \dd \vzeta(t)&=P_{\vzeta}\Big(\underbrace{\frac{1}{\sqrt{B}} \partial \Phi(\vzeta) \mSig^{1/2}(\vzeta)\dd \vW(t)}_{\text{(a)\ Diffusion}}\underbrace{-\frac{K}{2B}G(\vzeta) \dd t}_{\text{(b)\ Regularization}}\Big).
\end{align}
\begin{comment}
\begin{align}\label{eq: sde local sgd}
\begin{aligned}
    \dd \vzeta(t)&=\underbrace{\frac{1}{\sqrt{B}}\partial \Phi(\vzeta)\mSig^{1/2}(\vzeta)\dd \vW(t)-\frac{1}{2B}\nabla^2 \cL(\vzeta)^{+}\nabla^3\cL(\vzeta)\left[\mSig_{\parallel}(\vzeta)\right]\dd t}_{\text{(a)\ Diffusion\  Part}}\\
    &\quad \underbrace{-\frac{K}{2B}\partial \Phi(\vzeta)\nabla^3\cL(\vzeta)[\cV_{\nabla^2 \cL(\vzeta)}(\mSig_{\Diamond}(\vzeta))]\dd t}_{\text{(b) Regularization\  Part}}.
\end{aligned}
\end{align}
\end{comment}

This form establishes two basic components of the limiting SDE: the diffusion part and the regularization part.  
%The diffusion part consists of two terms where the former is the Brownian motion in the tangent space and the latter lives in the normal space, serving as a correction to pull the stochastic process back to the manifold. 
The diffusion part is the Brownian motion on $\Gamma$ while the regularization part can be viewed as the negative the gradient  of $\inner{\nabla^2 \cL(\vzeta)}{\cV_{\nabla^2 \cL(\vzeta)}(\mSig_{\Diamond}(\vzeta)) }$ projected onto the tangent space, but ignoring the dependency of $\cV_{\nabla^2 \cL(\vzeta)}(\mSig_{\Diamond}(\vzeta))$ on $\vzeta$. This can be connected to the class of semi-gradient methods which only computes a part of the gradient \citep{mnih2015human, DBLP:books/lib/SuttonB98, DBLP:conf/iclr/BrandfonbrenerB20}.

Note that the regularization part
reveals a deterministic trend towards the region with smaller magnitude of Hessian, which is commonly believed to correlate with better generalization \citep{hochreiter1997flat, keskar2017on, neyshabur2017exploring}. In contrast,  the diffusion part can be  regarded as random perturbation to this trend. Hence, we conjecture that \emph{a larger regularization term} or \emph{a smaller diffusion term} is beneficial to generalization. This view identifies the effect of different components of the noise covariance on generalization and therefore, goes one step further on the conventional wisdom that the magnitude of noise matters for generalization \citep{smith2020generalization, jastrzkebski2017three, keskar2017on}.

Comparing~\eqref{eq: sde sgd} and \eqref{eq: sde local sgd}, we observe that Local SGD amplifies the regularization part to $K$ times that of SGD, which may account for its improvement of generalization upon SGD.  Since the magnitude of the regularization part increases with $H\eta$, our conjecture also implies that we should increase the number of local steps when decreasing the learning rate to  experience similar generalization benefit from the regularization part, which coincides with the experimental results in \Cref{fig:effect} (e) and (f). 


To  justify the latter part of our conjecture, we conduct the following experiment where we keep $H$ and $\eta$ fixed and gradually increase the number of workers $K$ to reduce the diffusion part, or equivalently, enlarge the relative strength of the regularization part. As shown in \xinran{TBA} and Table \xinran{TBA}, a higher test is achieved for larger $K$. 
\begin{figure}[t]
\vspace{-0.5in}
\begin{center}
 \subfigure[CIFAR-10, $H=600$ for $K>1$.]{
        \includegraphics[width=0.4\textwidth]{figs/diffusion_cifar_shao}    }
    \hspace{0.1in}
         \subfigure[ImageNet, $H=78$ for $K>1$.]{
        \includegraphics[width=0.4\textwidth]{figs/img_diff}
    }
    \vspace{-0.1in}
        \caption{A smaller leads to better generalization. Test accuracy improves as we increase $K$ with fixed $\eta$ and $H$ to reduce the diffusion term while keeping the generalization part untouched. 
        See Appendix \xinran{TBA} for training details. }
      .   \label{fig:diffusion}
     \vspace{-0.2in}
\end{center}
\end{figure}

==> setup.tex <==
\section{TO BE REMOVED: Local SGD and Post-Local SGD}\label{sec:setup}

% \kaifeng{maybe we should not use the term "parallel SGD", because it refers to an algorithm that involves multiple workers.}

In this section, we formally introduce SGD, parallel SGD, Local SGD~\citep{???}, and Post-Local SGD~\citep{lin2020dont}.
%and set up necessary notations.

Gradient descent is an iterative method that optimizes a given loss function $\cL(\vtheta)$
by moving along the negative gradient direction in each step.
The update rule can be written as $\vtheta_{t+1} \gets \vtheta_t - \eta \vg_t$,
where
$\vg_t$ is either the accurate value or an estimate of the gradient of $\cL$ at $\vtheta_t$,
and $\eta$ is the learning rate.
In large-scale training,
it is more preferable to use stochastic gradient estimates,
because the exact computation of the gradients
typically requires a full scan over the dataset,
but a stochastic estimate can be obtained by just averaging over a mini-batch.
When $\vg_t$ is a stochastic gradient estimate,
we call the method as \textit{Stochastic Gradient Descent (SGD)} in particular.

For the purpose of theoretical analysis, we abstract the stochastic gradient estimate
as being provided by a \textit{noisy gradient oracle} $\cG_B$.
More formally, 
given a parameter vector $\vtheta$ as input,
$\cG$ draws a batch of $B$ independent samples from the dataset
and returns the average gradient at $\vtheta$ over the batch.
We denote $\cG_B(\vtheta)$ as the distribution of the oracle output at $\vtheta$.
%This gradient estimate is unbiased, i.e., 
%$\E_{\vg \sim \cG(\vtheta)}[\vg] = \nabla \cL(\vtheta)$.
SGD with batch size $B$ is then defined as an iterative method that performs the following updates:
\begin{equation} \label{eq:sgd}
    \vtheta_{t+1} \gets \vtheta_t - \eta \vg_t, \quad \vg_t \sim \cG_B(\vtheta_t).
\end{equation}
A practical implementation of SGD in distributed settings is \textit{parallel SGD}.
It is mathematically equivalent to SGD~\eqref{eq:sgd}, but the computation of stochastic gradient estimates
is distributed among $K \ge 2$ workers.
More specifically, 
in every step of training,
parallel SGD samples a batch of $B$ independent samples from the dataset,
and partitions the batch equally into $K$ local batches among the $K$ workers.
Each local batch thus has size $\Bloc := B / K$, referred as \textit{local batch size}.
To compute $\vg_t \sim \cG_B(\vtheta_t)$ in~\eqref{eq:sgd},
every worker first computes the average gradient over its local batch,
resulting in $K$ local gradients $\vg_{1,t}, \dots, \vg_{K, t}$,
then they average the local gradients through one round of communication
to obtain the final estimate $\vg_t \gets \frac{1}{K} \sum_{k=1}^{K}\vg_{k, t}$.

%resulting in $K$ local gradients $\vg_{1,t}, \dots, \vg_{K, t}$.
%Finally, the workers communicate with each other to average the local gradients $\vg_t \gets \frac{1}{K} \sum_{k=1}^{K}\vg_{k, t}$.

\begin{comment}
In this paper, we abstract the stochastic gradient estimate
as being provided by a \textit{noisy gradient oracle} $\cG$.
More formally, 
given a parameter vector $\vtheta$ as input,
$\cG$ draws a gradient estimate $\vg$
from a distribution depending on $\vtheta$, which we denote as $\cG(\vtheta)$.
We require the gradient estimate to be unbiased, i.e., $\E_{\vg \sim \cG(\vtheta)}[\vg] = \nabla \cL(\vtheta)$.
%$\cG$ is characterized by a distribution $\cG(\vtheta)$ parameterized by $\vtheta$.
%tuple $(\cL, \cZ)$,
%where $\cL(\vtheta)$ is the loss function and $\cZ(\vtheta)$ is a noise distribution depending on $\vtheta$.
When the gradient oracle is implemented by taking the gradient over a random batch of size $B$,
we use the symbol $\cG_{B}$ to emphasize the batch size.
Then SGD with batch size $B$ is defined as an iterative method that performs the following updates:
\begin{equation} \label{eq:sgd}
    \vtheta_{t+1} \gets \vtheta_t - \eta \vg_t, \quad \vg_t \sim \cG_B(\vtheta_t).
\end{equation}
A practical implementation of SGD in distributed settings is \textit{parallel SGD},

which involves multiple workers
to work together to compute stochastic gradient estimates over large batches.
More specifically,
parallel SGD assumes $K \ge 2$ workers sharing a common training set.
In each step, a batch of size $B$
is drawn either with or without replacement,
and is then split into $K$ smaller batches of size $\Bloc := B / K$,
each of which is sent to one client.
Then every client computes the average gradient over its local batch,
resulting in $K$ local gradients.
Finally, the workers communicate with each other to compute $\vg_t$
as the average over the $K$ local gradients, and perform the update $\vtheta_{t+1} \gets \vtheta_t - \eta \vg_t$.

Formally, we define $\cG$ as a noisy gradient oracle and abstract the local gradients
computed by each client as being provided by $\cG$.
Then the update rule of parallel SGD is as follows,
\begin{equation} \label{eq:parallel-sgd}
    \vtheta_{t+1} \gets \vtheta_t - \frac{\eta}{K} \sum_{k=1}^{K} \vg_{k,t},\quad\text{where}\quad\vg_{k,t} \sim \cG(\vtheta_t).
\end{equation}
\end{comment}
To fully utilize the hardware,
the local batch size $\Bloc$ should not be too small,
and thus
parallel SGD is expected to yield better speedups
when the batch size $B$ gets larger.
%in large-batch training,
%i.e., training the model with a large total batch size.
However, as mentioned in the introduction,
large-batch training suffers from two major problems:
high communication cost and degradation in generalization.

%However, as small-batch training with a single machine
%is always an alternative,
%several training tricks need to be deployed
%in large-batch training to make it 
%equally competitive as small-batch training.
%First,
%increasing the total batch size
%leads to fewer update steps in training
%the total number of SGD steps decreases
%as the batch size increases,
%when the total number of epochs is fixed.
%two major issues need to be addressed
%to make large-batch training
%do training with a large total batch size
%in presence of multiple physical machines.
%Parallel SGD is more effective in large-batch training.
%Parallel SGD
%Note that the speedup of Parallel SGD over the single-client SGD
%is better exhibited when the total batch size is large.
%the total batch size $B$ should be proportional to $K$.
%To allow Parallel SGD to achieve a linear speedup
%over SGD with the same total batch size $B$ as $K$ increases,
%can achieve a genuine speedup
%only if the total batch size is large enough;
%otherwise other factors such as data loading 
%the computation costs due to
%communication and I/O can
%be the dominating factors.
%local batch size $\Bloc$ is above some threshold (e.g., 32),
%since communication and I/O can introduce computational overhead
%\kaifeng{reword this?}.
%Therefore, it is necessary to set the total batch size $B$
%to be large to obtain a linear speedup as $K$ increases.

%\kaifeng{why parallel SGD is associated with large-batch training; the issues of large-batch training; how LSR leads to real speedups}

\begin{comment}
Each client receives one 
each client samples a mini-batch of $\Bloc$ data points (with or without replacement)
and computes the average gradient over its own mini-batch,
resulting in $K$ mini-batches and $K$ local gradients in total.
Then the workers communicate with each other to compute $\vg_t$
as the average over the $K$ local gradients, and finally perform the update $\vtheta_{t+1} \gets \vtheta_t - \eta \vg_t$.
\end{comment}

%gradient over all $K \cdot \Bloc$ samples from different workers.
%and compute
%sharing the same training set.
%In each step, every client 
%and these $K$ workers work jointly to compute the gradient in each step.
%More specifically, each 
%a distributed optimization method
%that aims to speed up SGD by letting $K$ workers work jointly
%to compute the stochastic gradient estimate.
\begin{comment}
aims to speed up SGD by leveraging data parallelism.
\kaifeng{search in the literature to find out a better way to say it}
Assume that there are $K$ workers that can access the oracle $\cG$.
In each step of Parallel SGD, each client
obtains a gradient estimate $\vg_{k, t} = \nabla \cL(\vtheta_t) + \vz_{k,t}$ independently
and uses the average gradient estimate to update the parameter.
\begin{equation} \label{eq:parallel-sgd}
    \vtheta_{t+1} \gets \vtheta_t - \frac{\eta}{K} \sum_{k=1}^{K} (\nabla \cL(\vtheta_t) + \vz_{k,t}), \quad \vz_{k,t} \sim \cZ(\vtheta_t).
\end{equation}
\kaifeng{explain how LSR leads to real speedups}
\end{comment}


\begin{comment}
These stochastic estimates are typically obtained by averaging over mini-batches,
but here we abstract them as being provided by a \textit{noisy} oracle $\cG$.

stochastic estimates of the gradients.

We study the optimization process of a loss function $\cL(\vtheta)$
with first-order 

We assume a loss function $\cL(\vtheta)$ which corresponds to
the average loss over the dataset.
In large-scale training, 
the exact loss values and gradients of $\cL(\vtheta)$ can be inefficient to compute,
and it is thus more preferable to

optimize the loss function given only the access to stochastic estimates.

use an algorithm that 

To circumvent this issue,

As the exact loss values and exact gradients are usually inefficient
to compute for large-scale datasets,

it is more preferable to use SGD, 

For large-scale training,

In this scenario,
SGD is proposed to optimize $\cL(\vtheta)$
given only the access to some stochastic estimates of the gradients.
These stochastic estimates are typically obtained by averaging over mini-batches,
but here we abstract them as being provided by a \textit{noisy} oracle $\cG$.
More formally, $\cG$ is characterized by a tuple $(\cL, \cZ)$,
where $\cL(\vtheta)$ is the loss function and $\cZ(\vtheta)$ is a noise distribution depending on $\vtheta$.
Given a parameter vector $\vtheta$ as input,
$\cG$ produces a gradient estimate $\vg = \nabla \cL(\vtheta) + \vz$, where $\vz \sim \cZ(\vtheta)$ is zero-mean noise sampled from $\cZ(\vtheta)$.
We define SGD as an iterative method that performs gradient descent using these gradient estimates.
\begin{equation} \label{eq:sgd}
    \vtheta_{t+1} \gets \vtheta_t - \eta (\nabla \cL(\vtheta_t) + \vz_t), \quad \vz_t \sim \cZ(\vtheta_t).
\end{equation}
\end{comment}

%aims to speed up the training
%by leveraging data parallelism
%In presence of multiple workers,
%= (\Loss, \mSigma, \cZ)$.
%which outputs a stochastic estimate of $\nabla \cL(\vtheta)$ once $\vtheta$ is given.
%a set of loss functions $\{ \ell_i(\vtheta) \}_{i \in \cI}$,
%where $\cI$ is the index set,
%Consider a dataset $\{ (\vx_i, y_i)\}$, where $\vx_i$ and $y_i$
%denote the input and target respectively.
%Let $f_i(\vtheta)$ be the output of the neural network
%on input $\vx_i$.
%we define $\{ \cL_i(\vtheta) \}_{i \in \cI}$
%to be the loss functions of $\vtheta$ indexed by $i \in \cI$.

\textit{Local SGD} can be seen as a generalization of parallel SGD to reduce communication cost.
The training process proceeds in rounds, % and
%produces a sequence of {\em global iterates} $\vths[0], \vths[1], \vths[2], \dots$,
where each round produces a global iterate $\vths$.
The round $s+1$ specifically works as follows.
%At round $s+1$, a new global iterate $\vths[s+1]$ is produced from $\vths$ as follows.
First, 
every worker $k \in [K]$ performs $H$ steps of SGD independently, starting with its local copy of the global iterate $\bvths$:
%where each round produces a \textit{global iterate} $\vths[s]$.
%produces a sequence of \textit{global iterates} $\bvths[0], \bvths[1], \bvths[2], \dots$,
%where the $s$-th round produces $\bvths$.
%Formally, every client $k$ at round $s$,
\begin{align}
    \vths_{k,0} &\gets \bvths, \\
    \vths_{k,t+1} &\gets \vths_{k, t} - \eta \vgs_{k, t}, \quad \text{where} \quad
    \vgs_{k, t} \sim \cG_{\Bloc}(\vths_{k, t}) \quad \text{for all } 0 \le t < H.
\end{align}
\kaifeng{emphasize independence}

After that,
%At the end of each round,
the workers perform an \textit{aggregation step} jointly
to compute the average of the resulting local iterates,
and the round ends by assigning the next global iterate as this average iterate:
$\bvths[s+1] \gets \frac{1}{K}\sum_{k=1}^K \vths_{k, H}$.

In the special case of $H=1$, Local SGD is equivalent to Parallel SGD,
since averaging the iterates in each step is equivalent to doing SGD with averaged gradients.

\textit{Post-local SGD} is a hybrid method proposed by \citet{lin2020dont}. It
starts training with parallel SGD and then switches to Local SGD with $H > 1$
after $t_0$ steps, where $t_0$ is called the \textit{post-local switching time}.
The gradient oracle $\cG_{\Bloc}$ and the number of workers $K$ are kept the
same after the switching. By adjusting the post-local switching time $t_0$, one
can trade off between parallel SGD and Local SGD (setting $t_0 = 0$ gives Local
SGD and setting $t_0 = +\infty$ gives parallel SGD).
%sometimes leading to better generalization than using SGD alone~\citep{lin2020dont}.

\myparagraph{Discrepancy with Practical Implementations.} All the above algorithms can add a momentum term for better performance, but our theoretical analysis will focus on the ones without momentum.
\kaifeng{also discuss with/without replacement}

%It is natural to change the value of $H$ in different phases of training.
%In this paper, we define \textit{Post-Local SGD} as Local SGD
%that assigns $H$ to $H_1 = 1$ in the beginning
%and then changes it to a fixed value $H_2 > 1$ after several rounds.
%Finally, the new global iterate $\bvths[s+1]$ is generated by taking the average over all resulting local iterates.
%proceeds in rounds. We use $\vths_{k,t}\in \R^d$ to denote the local iterate at round $s$ , step $t$ on device $k$ and $\bvths$ to denote the global iterate at the beginning of round $s$. We use $\Bloc$ and $B$ to denote the local batch size and global batch size respectively and $B=K\Bloc$. At the beginning of round $s$, each client sets the local iterate as the global iterate, that is, 
%\begin{align*}
%      \vths_{k,0} &= \bvths, &\forall k \in [K].
%\end{align*}
%where $\vzs_{k, t}$ is the gradient noise with mean zero and covariance $\frac{1}{\Bloc}\mSig(\vths_{k, t})$.

